Atomic RMI 2: Highly Parallel Pessimistic Distributed Transactional Memory

Distributed Transactional Memory (DTM) is an emerging approach to distributed synchronization based on the application of the transaction abstraction to distributed computation. DTM comes in several system models, but the control flow model (CF) is particularly powerful, since it allows transactions to delegate computation to remote nodes as well as access shared data. However, there are no existing CF DTM systems that perform on par with state-of-the-art systems operating in other models. Hence, we introduce a CF DTM synchronization algorithm, OptSVA-CF. It supports fine-grained pessimistic concurrency control, so it avoids aborts, and thus avoids problems with irrevocable operations. Furthermore, it uses early release and asynchrony to parallelize concurrent transactions to a high degree, while retaining strong safety properties. We implement it as Atomic RMI 2, in effect producing a CF DTM system that, as our evaluation shows, can outperform a state-of-the-art non-CF DTM such as HyFlow2.

==> optsva-cf-alg.tex <==
%
%
%
    \begin{lstlisting}[name=optsva]
procedure start(Transaction $\trobj_i$) {
  for($\objx$ ∈ $\accesses{i}$ sorted by $\prec_\lockf$)
    lock $\lock{\objx}$
  for($\objx$ ∈ $\accesses{i}$) {
    $\gv{\objx}$ ← $\gv{\objx}$ + 1
    $\pv{\objx}{i}$ ← $\gv{\objx}$
  }
  for($\objx$ ∈ $\accesses{i}$ sorted by $\prec_\lockf$)
    unlock $\lock{\objx}$
  for($\objx$ ∈ $\accesses{i}$: $\objx$ is read-only)
    async run read_buffer($\trobj_i$,$\objx$)
      when $\pv{\objx}{i}$ - 1 = $\lv{\objx}$
}
    \end{lstlisting}
\makeatletter
\lstset{linebackgroundcolor=%
  %
  firstnumber=auto, 
}
\csname\@lst @SetFirstNumber\endcsname
\makeatother
\begin{lstlisting}[name=optsva]
procedure read(Transaction $\trobj_i$, TObj $\objx$, Method $\method$) {
  // Read-only object.
  if ($\objx$ is read-only) {                    
    join with read_buffer($\trobj_i$,$\objx$)   
    execute $\method$ on $\buf{i}{\objx}$ returning $\val$
    $\rc{i}{\objx}$ ← $\rc{i}{\objx}$ + 1
    return $\val$
  }
  // Object not previously released.
  if ($\wc{i}{\objx}$ < $\wub{i}{\objx}$ or $\uc{i}{\objx}$ < $\uub{i}{\objx}$) { 
    if ($\wc{i}{\objx}$ = 0 and $\uc{i}{\objx} = 0$) {                       
      wait until $\pv{\objx}{i}$ - 1 = $\lv{\objx}$  
      checkpoint($\trobj_i$,$\objx$)
      if ($\wc{i}{\objx}$ > 0)                           
        apply $\log{i}{\objx}$ to $\objx$         
    }
    if (∃$\objy$: $\rv{i}{\objy}$ = $\cv{\objy}$)
      abort($\trobj_i$) and exit
    execute $\method$ on $\objx$ returning $\val$
    $\rc{i}{\objx}$ ← $\rc{i}{\objx}$ + 1                 
    if ($\rc{i}{\objx}$ = $\rub{i}{\objx}$ and $\wc{i}{\objx}$ = $\wub{i}{\objx}$ 
         and $\uc{i}{\objx}$ = $\uub{i}{\objx}$) 
      release($\trobj_i$,$\objx$)        
    return $\val$
  }
  // Object previously released.
  if ($\wc{i}{\objx}$ = $\wub{i}{\objx}$ and $\uc{i}{\objx}$ = $\uub{i}{\objx}$) { 
    if (write_bufferd($\trobj_i$,$\objx$) is running)   
      join with write_buffer($\trobj_i$,$\objx$)     
    execute $\method$ on $\buf{i}{\objx}$ returning $\val$
    $\rc{i}{\objx}$ ← $\rc{i}{\objx}$ + 1
    return $\val$
  } 
}
\end{lstlisting}


%
%
%
%
%
%
%
%
%
%
%
%
\makeatletter
\lstset{linebackgroundcolor=%
  firstnumber=auto, 
}
\csname\@lst @SetFirstNumber\endcsname
\makeatother
\begin{lstlisting}[name=optsva]
procedure update(Transaction $\trobj_i$, TObj $\objx$, Method $\method$) {
  if ($\rc{i}{\objx}$ = 0 and $\uc{i}{\objx}$ = 0) {
    wait until $\pv{\objx}{i}$ - 1 = $\lv{\objx}$
    checkpoint($\trobj_i$,$\objx$)
    if ($\wc{i}{\objx}$ > 0)
      apply $\log{i}{\objx}$ to $\objx$
  }
  execute $\method$ on $\obj$ returning $\val$
  $\uc{i}{\objx}$ ← $\uc{i}{\objx}$ + 1
  if ($\wub{i}{\objx}$ = $\wc{i}{\objx}$ and $\uub{i}{\objx}$ = $\uc{i}{\objx}$) {
    copy $\obj$ to $\buf{i}{\objx}$
    release($\trobj_i$,$\objx$)
  }
  return $\val$
}
\end{lstlisting}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\makeatletter
\lstset{linebackgroundcolor=%
    firstnumber=auto, 
}
\csname\@lst @SetFirstNumber\endcsname
\makeatother
\begin{lstlisting}[name=optsva]
procedure write(Transaction $\trobj_i$, TObj $\objx$, Method $\method$) {
  // No preceding reads or updates.
  if ($\rc{i}{\objx}$ = 0 and $\uc{i}{\objx}$ = 0) {
      execute $\method$ on $\log{i}{\objx}$ returning ${\tt nothing}$
    $\wc{i}{\objx}$++
    if ($\wc{i}{\objx}$ = $\wub{i}{\objx}$)
      async run write_buffer($\trobj_i$,$\objx$)
        when $\pv{\objx}{i}$ - 1 = $\lv{\objx}$
  } 
  // Some preceeding reads or updates. 
  if ($\rc{i}{\objx}$ > 0 or $\uc{i}{\objx}$ > 0) {
    if (∃$\objy$: $\rv{i}{\objy}$ = $\cv{\objy}$)
      abort($\trobj_i$) and exit 
      execute $\method$ on $\objx$ returning ${\tt nothing}$
    $\wc{i}{\objx}$ ← $\wc{i}{\objx}$ + 1
    if ($\wc{i}{\objx}$ = $\wub{i}{\objx}$) {
      copy $\objx$ to $\buf{i}{\objx}$
      release($\trobj_i$,$\objx$)
    }
  }    
}
\end{lstlisting}
%
%
%
%
%
%
%
%
%
%
%
\begin{lstlisting}[name=optsva]
procedure commit(Transaction $\trobj_i$) {
  for($\objx$ ∈ $\accesses{i}$) {
    if ($\objx$ is read-only)
      join with read_comit($\trobj_i$,$\objx$)
    else {
      if ($\wc{i}{\objx}$ = $\wub{i}{\objx}$ 
           and $\rc{i}{\objx}$ = 0 
           and $\uc{i}{\objx}$ = 0) 
        join with write_buffer($\trobj_i$,$\objx$)
      else
        catch_up($\trobj_i$, $\objx$)
      wait until $\pv{\objx}{i}$ - 1 = $\ltv{\objx}$
      if ($\pv{\objx}{i}$ - 1 = $\lv{\objx}$)
        $\lv{\objx}$ ← $\pv{\objx}{i}$
      if ($\rc{i}{\objx}$ + $\wc{i}{\objx}$ + $\uc{i}{\objx}$ > 0
           and $\rv{i}{\objx}$ = $\cv{\objx}$
           and $\pv{\objx}{i}$ - 1 > $\lv{\objx}$)
        $\cv{\objx}$ ← $\pv{\objx}{i}$
    }
  }
  if (∃$\objy$: $\rv{i}{\objy}$ > $\cv{\objy}$) 
    abort($\trobj_i$) and exit
  for($\objx$ ∈ $\accesses{i}$)
    $\ltv{\objx}$ ← $\pv{\objx}{i}$
}
\end{lstlisting}

%
%
%
%
%
%
%
\begin{lstlisting}[name=optsva]
procedure abort(Transaction $\trobj_i$) {
  for($\objx$ ∈ $\accesses{i}$) { 
    wait until $\pv{\objx}{i}$ - 1 = $\ltv{\objx}$
    if ($\rc{i}{\objx}$ + $\wc{i}{\objx}$ + $\uc{i}{\objx}$ > 0 
         and $\pv{\objx}{i}$ - 1 > $\lv{\objx}$ 
         and $\rv{i}{\objx}$ = $\cv{\objx}$ 
         and $\objx$ is not read-only) {
      if ($\wc{i}{\objx}$ = $\wub{i}{\objx}$)                                           
        join with write_buffer($\trobj_i$,$\objx$)
      recover($\trobj_i$,$\objx$)
    }
    if ($\pv{\objx}{i}$ - 1 = $\lv{\objx}$)
      $\lv{\objx}$ ← $\pv{\objx}{i}$
    $\ltv{\objx}$ ← $\pv{\objx}{i}$
  }
}
\end{lstlisting}

\makeatletter
%
%
%
%
\csname\@lst @SetFirstNumber\endcsname
\makeatother
\begin{lstlisting}[name=optsva]
procedure read_buffer(Transaction $\trobj_i$, TObj $\objx$) {
  $\rv{i}{\objx}$ ← $\cv{\objx}$ 
  copy $\objx$ to $\buf{i}{\objx}$
  release($\trobj_i$,$\objx$) 
  async run read_commit($\trobj_i$,$\objx$)
    when $\pv{\objx}{i}$ - 1 = $\ltv{\objx}$
}
procedure read_commit(Transaction $\trobj_i$, TObj $\objx$) {
  $\cv{\objx}$ ← $\pv{\objx}{i}$ 
  if (∃$\objy$: $\rv{i}{\objy}$ > $\cv{\objy}$)
    abort($\trobj_i$) and exit
  $\ltv{\objx}$ ← $\pv{\objx}{i}$ 
}
procedure write_buffer(Transaction $\trobj_i$, TObj $\objx$) { 
  checkpoint($\trobj_i$,$\objx$)
  apply $\log{i}{\objx}$ to $\objx$
  copy $\objx$ to $\buf{i}{\objx}$
  release($\trobj_i$,$\objx$)
}
procedure checkpoint(Transaction $\trobj_i$, TObj $\objx$) {
  copy $\objx$ to $\stored{i}{\objx}$
  $\rv{i}{\objx}$ ← $\cv{\objx}$
}
procedure recover(Transaction $\trobj_i$, TObj $\objx$) {
  revert $\objx$ from $\stored{i}{\objx}$
  $\cv{\objx}$ ← $\rv{i}{\objx}$
}
procedure release(Transaction $\trobj_i$, TObj $\objx$) {
  $\cv{\objx}$ ← $\pv{\objx}{i}$
  $\lv{\objx}$ ← $\pv{\objx}{i}$
}
procedure catch_up(Transaction $\trobj_i$, TObj $\objx$) {
  if ($\wc{i}{\objx}$ = 0 and $\rc{i}{\objx}$ = 0 
       and $\uc{i}{\objx}$ = 0) 
    wait until $\pv{\objx}{i}$ - 1 = $\lv{\objx}$
  if ($\wc{i}{\objx}$ > 0 and $\rc{i}{\objx}$ = 0 
       and $\uc{i}{\objx}$ = 0) {
    checkpoint($\trobj_i$,$\objx$)
    apply $\log{i}{\objx}$ to $\objx$
  }
}
\end{lstlisting}

